A Relation Algebra for Term Rewriting: A differential approach to sequential reduction (Revised Version)

Recently, Gavazzo has developed a relational theory of symbolic manipulation, that allows to study syntax-based rewriting systems without relying on specific notions of syntax. This theory was obtained by extending the algebra of relations with syntax-inspired operators. Within the algebras thus obtained, it is possible to encode notions of parallel and full reduction for first-order rewriting systems, as well as to prove nontrivial properties about them in an algebraic and syntax-independent fashion. Sequential reduction, however, was not explored, but it was conjectured that it could be studied through a differential relational theory of rewriting. This manuscript proves the above conjecture by defining differential algebras of term relations, viz. algebras of term relations extended with novel operators inspired by the theory of functor derivatives. We give a set of axioms and rules for such operators and show that the resulting theory is expressive enough to define notions of parallel, full, and sequential reduction. We prove fundamental results relating all these notions in a purely algebraic and syntax-independent way, and showcase the effectiveness of our theory by proving the soundness of a proof technique for weak confluence akin to the so-called Critical Pair Lemma.

==> figures/algebraic_laws.tex <==
\begin{figure}
  \centering
  \footnotesize
\begin{framed}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \begin{align*}
            \bot &\leq a
            \\
            a &\leq \top
            \\
            \bigvee a_i \leq b &\iff
            \forall i.\ a_i \leq b
            \\
            b \leq \bigwedge a_i &\iff \forall i.\ b \leq a_i
            \\
             a; \Delta &= a
            \\
            \Delta;a &= a
            \\
            a; (b; c) &= (a; b);c
        \end{align*}
         \caption{Lattice and monoid laws}
         \label{fig:algebraic-laws-lattice}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.4\textwidth}
         \centering
            \begin{align*}
                a;\bot &= \bot 
                \\
                \bot; a &= \bot
                \\
                a; \Big(\bigvee_i b_i\Big) &= \bigvee_i (a;b_i)
                \\
                \Big(\bigvee_i a_i \Big); b &= \bigvee_i (a_i;b)
                \\
                a_1 \leq b_1 \,\,\&\,\, a_2 \leq b_2 
                &\implies a_1;a_2 \leq b_1;b_2
            \end{align*}         
        \caption{Quantale Laws}
         \label{fig:algenbraic-laws-quantale}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
            \begin{align*}
            a\op \leq b \iff& a \leq b\op
            \\
            \Delta\op &= \Delta
            \\
            \bot\op &= \bot
            \\
            \top\op &= \top
            \\
            a\op &= a
            \\
            (a;b)\op &= b\op; a\op
            \\
            \Big(\bigvee a_i\Big)\op &= \bigvee a_i\op
        \end{align*}
        \caption{Converse Laws}
         \label{fig:algebraic-laws-converse}
     \end{subfigure}
\end{framed}
        \caption{Algebraic Laws}
        \label{fig:algebraic-laws}
\end{figure} 

